From Occurrence to Consequence: A Comprehensive Data-driven Analysis of Building Fire Risk

Building fires pose a persistent threat to life, property, and infrastructure, emphasizing the need for advanced risk mitigation strategies. This study presents a data-driven framework analyzing U.S. fire risks by integrating over one million fire incident reports with diverse fire-relevant datasets, including social determinants, building inventories, weather conditions, and incident-specific factors. By adapting machine learning models, we identify key risk factors influencing fire occurrence and consequences. Our findings show that vulnerable communities, characterized by socioeconomic disparities or the prevalence of outdated or vacant buildings, face higher fire risks. Incident-specific factors, such as fire origins and safety features, strongly influence fire consequences. Buildings equipped with fire detectors and automatic extinguishing systems experience significantly lower fire spread and injury risks. By pinpointing high-risk areas and populations, this research supports targeted interventions, including mandating fire safety systems and providing subsidies for disadvantaged communities. These measures can enhance fire prevention, protect vulnerable groups, and promote safer, more equitable communities.

==> conclusion.tex <==
\section{Limitation}

This study has several limitations. First, to facilitate analysis, textual information from fire incident reports is converted into numerical inputs, potentially overlooking nuanced information embedded within the text. Future research can leverage large language models (LLMs) to capture the contextual and semantic richness of this textual data. Second, certain categorical features with numerous subcategories (e.g., location of fire origin, property usage) are aggregated into broader groups based on the NFIRS codebook to ensure consistency and analytical tractability. While necessary, this may have reduced granularity and masked subtle patterns within the original data. Finally, the analysis assumes complete reporting of fire events within each ZIP code in the dataset. While necessary for analysis, this assumption may affect the representativeness of data for specific regions. Further research can explore methods to address potential reporting biases and incorporate more granular categorical information to enhance the model's accuracy and interpretive power.

% \textbf{Text-to-Numerical Conversion.} To facilitate the analysis, all textual information from fire incident reports was converted into numerical inputs. While this approach streamlines data processing, it may overlook nuanced information embedded within the text. Future research could address this limitation by leveraging large language models (LLMs) to capture the contextual and semantic nature of textual data more effectively. 

% \textbf{Simplification of Categorical Features.} Certain categorical features in the dataset contain dozens of subcategories (for instance, location of fire origin include 87 distinct sub categories and property usage includes 156 sub categories). For simplicity and consistency, these were consolidated into broader groups based on the NFIRS codebook. While this grouping aids in analysis, it may reduce the granularity of certain insights, potentially masking subtle patterns within the original data.

% \textbf{Simplifying Assumptions About Reporting Completeness.} We assume that when a ZIP code appears in the our fire incident dataset, all fire events within that ZIP code area are reported. This assumption, while necessary to facilitate analysis, may affect the representativeness of data for certain regions.


% \textbf{Work to do:}
% \begin{itemize}
%     % \item Rewrite contribution (Genralize to disease spread): Hongru
%     % \begin{itemize}
%     %     \item Adapt text reasoning to disease spread learning with multi-modality data (RNN encoder)
%     %     % Multi modality disease spread learning as text reasoning
%     %     \item Response to real-time info(real-time + zero-shot, variant, policy)
%     %     % Real time pandemic information integration.
%     %     \item Trustworthy
%     %     % Reliable and trustworthy decision-making pipeline.
%     % \end{itemize}
%     \item Update abstract Hongru
%     \begin{itemize}
%         \item Mention short-term, real-time
%         \item Clear mention our target is hospitalization
%         \item Think about how to present our performance? Compare with baseline improvement. 
%         \item Highlight the value of genomic data
%         \item Highlight the value of RNN encoder (based on results from the ablation study)
%     \end{itemize}
%     \item Update intro Frank
%     \begin{itemize}
%         \item Include transmission dynamic models
%         \item highlight short-term and real-time
%     \end{itemize}
%     \item Aviod using interpretable in the paper (?aviod black-box?) Change to robust/trustworthy (All)
%     \item We may add a couple example prompts in appendix. (3 -5) Shaochong focus on changes
% \end{itemize}

% \section{\textcolor{red}{Check List}}
% \begin{itemize}
%     \item Figure 1a
%     \item All captions for tables and figures
%     \item Figure 2. Check the text in the prompt. 
%     \item Sections 3.3 and 3.6 need update after finalize the results
%     \item Check the equivalent figures of Fig.3 a,b with other error metrics; if good, we can add them to the appendix.
%     \item Decide whether to add additional figures like 4 and 5 with other error metrics in the appendix. 
%     \item Maybe remove table 2. 
%     \item 6 needs update (x-axis should follow the prediction target time.)
%     \item Figure 8 need an update
% \end{itemize}





==> extended_data.tex <==
\section{Extended Data}



==> reference.tex <==
\section{References} 

Please use numerical references only for citations, and include the references within the manuscript file itself.  If you wish to use BibTeX, please copy the reference list from the .bbl file, paste it into the main manuscript .tex file, and delete the associated \bibliography and \bibliographystyle commands. Before submission, please ensure that the complete .tex file compiles successfully on your own system with no errors or warnings. There is no need to spend time visually formatting the manuscript: our style will be imposed automatically when the paper is prepared for publication.\\

\noindent Please do not cite web sites in the reference list — these should be listed separately, with the URLs in the Related Links section (see below).  If you are unsure if the website is a ‘Related link’ or should go in the ‘References’ section then identify if there is a publication date on the website.  If there is a publication date, it is likely that the item will be in the ‘References’ section.  If there is no publication date, it is likely that the item will be in the ‘Related Links’ section.\\

\noindent When citing a book, please indicate if you are citing a specific page range or chapter.  Otherwise, we presume that you are citing the entire book.  \\

\noindent \textbf{Highlighted references (optional)} Please select 5–-10 key references and provide a single sentence for each, highlighting the significance of the work.\\

\noindent\textbf{Acknowledgements}\\
E.g. Funding agencies.\\

\noindent\textbf{Author contributions}\\
Please describe the contributions made by each author.  Please use the initials of the individual author to explain these contributions.  These contributions are also required when you upload the files to our submission website.\\

\noindent\textbf{Competing interests}\\
Nature Journals require authors to declare any competing interests in relation to the work described. Information on this policy is available \href{http://www.nature.com/authors/policies/competing.html}{here}. \\



\noindent\textbf{Supplementary information (optional)}
If your article requires supplementary information, please include these files for peer-review. Please note that supplementary information will not be edited.

\begin{thebibliography}{10}

\bibitem{Hartkens_MICCAI_2002}
Hartkens, T., Hill, D.L., Castellano-Smith, A.D., Hawkes, D.J., Maurer, C.R., Martin, A.J., Hall, W.A., Liu, H. and Truwit, C.L.: Using points and surfaces to improve voxel-based non-rigid registration. In MICCAI, pp. 565-572. (2002)

\bibitem{zheng2020gman}
Zheng C, Fan X, Wang C, Qi J. Gman: A graph multi-attention network for traffic prediction. InProceedings of the AAAI Conference on Artificial Intelligence 2020 Apr 3 (Vol. 34, No. 01, pp. 1234-1241).

\bibitem{yao2019revisiting}
Yao H, Tang X, Wei H, Zheng G, Li Z. Revisiting spatial-temporal similarity: A deep learning framework for traffic prediction. InProceedings of the AAAI conference on artificial intelligence 2019 Jul 17 (Vol. 33, No. 01, pp. 5668-5675).

Zhao L, Song Y, Zhang C, Liu Y, Wang P, Lin T, Deng M, Li H. T-gcn: A temporal graph convolutional network for traffic prediction. IEEE Transactions on Intelligent Transportation Systems. 2019 Aug 22;21(9):3848-58.

\bibitem{xu2020spatial}
Xu M, Dai W, Liu C, Gao X, Lin W, Qi GJ, Xiong H. Spatial-temporal transformer networks for traffic flow forecasting. arXiv preprint arXiv:2001.02908. 2020 Jan 9.

\end{thebibliography}



==> tables/GAM_data_description.tex <==

\renewcommand{\arraystretch}{1.3}
\begin{longtable}{>{\centering\arraybackslash}m{5cm} | >{\centering\arraybackslash}m{10cm} } 
 \caption{Final list of variables used in GAM analysis} \label{tab:gam_variable_description} \\
    \toprule[1.5pt]
    \textbf{Variable name} & \textbf{Variable description} \\
    \hline
    \endfirsthead
    \hline
    \textbf{Variable name} & \textbf{Variable description} \\
    \hline
    \endhead
    \hline
    \endfoot
    Urban population ratio & The proportion of populations live in areas identified as urban. \\
    \hline
    Bachelor or higher ratio & The proportion of the population holds a bachelor's or higher degree. \\
    \hline
    Age 62+ ratio & The proportion of the population with age larger than or equal to 62 years old. \\
    \hline
    Black population ratio & The proportion of population identified as Blacks. \\
    \hline
    Industrial & The proportion of  establishments with NAICS code 22 (Utilities), 23 (Construction), and 31-33 (Manufacturing) over all the establishments. \\
    \hline
    Transportation and storage & The proportion of business establishments with NAICS code 48-49 (Transportation and Warehousing), and 81 (Other Services) over all the establishments. \\
    \hline
    Occupied units ratio & The proportion of occupied building units among all the building units in the considered area (county or ZIP-code area). \\
    \hline
    Built after 1980 ratio & The proportion of  building units built after 1980. \\
    \hline
    Monthly temperature & The monthly average temperature in the considered area. \\
    \hline
    Palmer Z-Index & Short-term drought indicator that measures moisture anomalies on a monthly basis, with positive values indicating wetter-than-normal conditions.\\

\bottomrule[1.5pt]

\end{longtable}

==> tables/consequence_target.tex <==
\begin{longtable}{>{\centering\arraybackslash}m{3cm} | >{\centering\arraybackslash}m{7cm} | >{\centering\arraybackslash}m{4cm} } 
    \caption{Fire consequence targets and related variables} 
    \label{tab:consequence_target} \\
    \toprule[1.5pt]
    \textbf{Target Name} & \textbf{Related .DBF field name} & \textbf{Size of database}  \\
    \hline
    \endfirsthead
    \hline
    \textbf{Target Name} & \textbf{Related .DBF field name} & \textbf{Size of database} \\
    \endhead
    \hline
    \endfoot
    Fire spread & FIRE-SPRD & 672,338\\
    \hline
    Human injury & SEV-1, SEV-2, SEV-3, SEV-4, and SEV-5 &  34,074\\
    \hline
    Economic loss & PROP-LOSS and CONT-LOSS & 484,964 \\
    \bottomrule[1.5pt]
\end{longtable}

==> tables/consequence_variable.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{longtable}{>{\centering\arraybackslash}m{1cm} | >{\centering\arraybackslash}m{3cm} | >{\centering\arraybackslash}m{5cm} | >{\centering\arraybackslash}m{5cm} } 
    \caption{Full list of incident-specific factors used in fire consequence analysis} \label{tab:fire-report-features} \\
    \toprule[1.5pt]
    \textbf{\#} & \textbf{Variable Name} & \textbf{Variable Description} & \textbf{.DBF field name and calculation}\\
    \hline
    \endfirsthead
    \hline
    \textbf{\#} & \textbf{Variable Name} & \textbf{Variable Description} & \textbf{.DBF field name and calculation} \\
    \hline
    \endhead
    \hline
    \endfoot
    1 & Event index & Unique identifier for the fire incident. & INCIDENT-KEY\\
    \hline
    2 & State & State where the fire incident occurred. & STATE \\
    \hline
    3 & Cause of ignition & Cause of ignition for the fire. & CAUSE-IGN\\
    \hline
    4 & Stories above grade & Number of building stories above the ground. & BLDG-ABOVE\\
    \hline
    5 & Stories below grade & Number of building levels below the ground. & BLDG-BELOW\\
    \hline
    6 & Total square footage & Total square footage of the building that fire originate from. &  TOT-SQ-FT \\
    \hline
    7 & Fire origin & Story of the fire origin. & FIRE-ORIG \\
    \hline
    8 & Flame spread & Whether the flame spread observed (Yes or No).& FLAME-SPRD \\
    \hline
    9 & Detectors & Presence of fire detectors. & DETECTOR \\
    \hline
    10 & AES presence & Presence of Automatic Extinguishing Systems (AES). & AES-PRES \\
    \hline
    11 & Number of unit  & Number of units involved in the building. & NUM-UNIT \\
    \hline
    12 & Response time & Fire department response time in minutes. & Calculated by ARRIVAL minus ALARM \\
    \hline
    13 & Accident year & Year of the fire incident. & Extracted from ALARM\\
    \hline
    14 & Accident month & Month of the fire incident. & Extracted from ALARM \\
    \hline
    15 & Accident day & Day of the fire incident. & Extracted from ALARM \\
    \hline
    16 & Accident hour & Hour of the fire incident. & Extracted from ALARM \\
    \hline
    17 & Human factors & The human condition or situation that allowed the heat source and combustible material to combine to
ignite the fire. & Derived from HUM-FAC-1 to HUM-FAC-8 \\
    \hline
    18 & Location of fire origin & The primary use of the area where the fire started within the property. & Grouped based on AREA-ORIG \\
    \hline
    19 & Primary action taken & The duties performed at the incident scene by the responding fire department personnel. & Grouped based on ACT-TAK1 \\
    \hline
    20 & Factors contributing to ignition & The contributing factors that allowed the heat source and combustible material to combine to ignite the
fire. &  Grouped based on FACT-IGN1\\
    \hline
    21 & Heat source & The specific source of the heat energy that started the fire. & Grouped based on HEAT-SOUR \\
    \hline
    22 & Item first ignited & The use or configuration of the item or material first ignited by the heat source. & Grouped based on FIRST-IGN \\
    \hline
    23 & Type of Material & The composition of the material in the item first ignited by the heat source. & Grouped based on TYPE-MAT \\
    \hline
    24 & Property usage & The actual use of the property where the incident occurred. & Grouped based on  PROP-USE \\
    \hline
    25 & Suppression factor & Factors that contributed to the growth, spread, or suppression of the fire. & Grouped based on SUP-FAC-1 \\
    \hline
    26 & Item spread & The item contributing most to flame spread. & Grouped based on ITEM-SPRD  \\
    \hline
    27 & Material spread & The type of material contributing most to flame spread. & Grouped based on MAT-SPRD \\
    % \hline
    % 28 & Fire spread & Fire spread indicator. & FIRE-SPRD \\
    % \hline
    % 29 & Human injury & Risk category of human injuries due to fire. & Derived based on the OTH-INJ, OTH-DEATH, and SEVERITY, \\ 
    % \hline
    % 30 & Economic loss &  Risk category of Fire-related content and property losses. & Calculated by PROP-LOSS PLUSE CONT-LOSS and then adjusted to 2022 value \\
    \bottomrule[1.5pt]
\end{longtable}

\newpage

==> tables/consequence_variable_local.tex <==

\renewcommand{\arraystretch}{1.3}
\begin{longtable}{>{\centering\arraybackslash}m{1cm} | >{\centering\arraybackslash}m{5cm} | >{\centering\arraybackslash}m{9cm} } 
    \caption{Full list of local factors used in fire consequence analysis} 
    \label{tab:local-factors} \\
    \toprule[1.5pt]
    \textbf{\#} & \textbf{Variable Name} & \textbf{Variable Description} \\
    \hline
    \endfirsthead
    \hline
    \textbf{\#} & \textbf{Variable Name} & \textbf{Variable Description} \\
    \hline
    \endhead
    \hline
    \endfoot
    1 & Median income & Average annual median household income in the county or ZIP-code area of the fire incident. \\
    \hline
    2 & Median rent & Average monthly median rent value. \\
    \hline
    3 & Occupied units ratio & The proportion of occupied building units. \\
    \hline
    4 & Utility gas ratio & The proportion of households using utility gas. \\
    \hline
    5 & Disability ratio & The proportion of population with disabilities. \\
    \hline
    6 & Bachelor or higher ratio & The proportion of the population holds a bachelor or higher degree. \\
    \hline
    7 & Health insurance ratio & The proportion of population with health insurance coverage. \\
    \hline
    8 & Age 62+ ratio & The proportion of population aged 62 or older. \\
    \hline
    9 & Employment ratio & The proportion of labor force aged 16 and over who are employed. \\
    \hline
    10 & Temperature & Hourly temperature at the time of fire. \\
    \hline
    11 & Relative humidity & Hourly relative humidity at the time of fire. \\
    \hline
    12 & Wind speed & Hourly wind speed at the time of fire. \\
    \hline
    13 & Minority populations & The proportion of the population excluding White and Black individuals in the area. \\
    \hline
    14 & Black ratio & The proportion of population identified as Blacks. \\
    \hline
    15 & Built after 1980 ratio & The proportion of building units after 1980. \\
    \hline
    16 & Solar or no fuel & The proportion of building units using solar or no fuel for heating. \\
    \hline
    17 & Coal or wood & The proportion of building units using coal or wood for heating. \\
    \bottomrule[1.5pt]
\end{longtable}




